The Furstenberg Boundary of a Groupoid

We define the Furstenberg boundary of a locally compact Hausdorff \'etale groupoid, generalising the Furstenberg boundary for discrete groups, by providing a construction of a groupoid-equivariant injective envelope. Using this injective envelope, we establish the absence of recurrent amenable subgroups in the isotropy as a sufficient criterion for the intersection property of a locally compact Hausdorff \'etale groupoid with compact unit space and no fixed points. This yields a criterion for C*-simplicity of minimal groupoids.

==> files/intersection.tex <==
\section{Intersection Property of \Etale{} Groupoids}\label{sec:intersection}
We now set out to prove our main theorem:
\begin{theorem}
  Let $\G$ be a locally compact \etale{} Hausdorff groupoid 
  \comment{in which every orbit has at most two points}.
  Then $\G$ has the intersection property exactly if for every choice
  $\Lambda = \{\Lambda_u \mid u\in \G^{(0)}\}$ 
  of amenable subgroups $\Lambda_u\leq \G_u^u$ of the isotropy groups,
  the closure of the $\G$-orbit of $\Lambda$ 
  in the Chabauty space of $\text{Iso}(\G)\subseteq \G$ 
  contains $\left\{\{u\} \mid u\in \G^{(0)}\right\}$
  \label{thm:main}
  \par
  Moreover, if the action of $\G$ on it's unit space is minimal,
  the condition about non-stationary orbits is automatically satisfied
  and $\Csr(\G)$ will be simple exactly if $\G$ satisfies the condition above.
\end{theorem}

In the spirit of Kalantar--Kennedy \cite{KennedyBoundaries}, 
Ozawa \cite{FurstenbergBoundaryLecture} and Kawabe \cite{Kawabe},
we will 
from the given groupoid $\G$
construct a second, nicer groupoid $\tilde \G$
for which the intersection property coincides with being principal
and which will have the intersection property exactly if $\G$ does.

In particular, we consider the action of $\G$ on it's unit space $X$
and form the $\G$-equivariant injective envelope $C(\tilde X)$ of $C(X)$ as described above.
Since $\G$ acts on $C(\tilde X)$ and therefore on $\tilde X$,
we may consider the transformation groupoid $\tilde \G \defeq \G \ltimes \tilde X$,
in analogy to Kawabe's proof.
As $\tilde X$ will turn out to be Stonean,
the isotropy of $\tilde \G$ will, under some weak assumptions,
be open 
and hence topological principality and principality coincide.

\begin{lemma}
  There is a canonical embedding
  $\Csr(\G) \hookrightarrow \Csr\left( \tilde \G \right)$.
  \label{lem:reducedAlgebraEmbeds}
\end{lemma}
\begin{proof}
  We denote by $q\colon \tilde X \rightarrow X$ the quotient map 
  that comes associated with taking the $\G$-equivariant injective envelope.
  As a set, $\tilde \G$ is 
  $\left\{ (\gamma, \tilde x) \bigm | \gamma \in \G, \tilde x \in \tilde X, r(\gamma) 
  = q(\tilde x) \right\}$
  and the range and source maps are given by 
  $r\left( (\gamma, \tilde x) \right) = \tilde x$
  and
  $s\left( (\gamma, \tilde x) \right) = \gamma^{-1}.\tilde x$.
  We also denote by $Q\colon \tilde \G \rightarrow \G$ the groupoid homomorphism given by
  $(\gamma, \tilde x) \mapsto \gamma$, which extends $q\colon \tilde X \rightarrow X$.
  \todocomment{Do we need to explain that we get a $\G$-action on $\tilde X$
  by shifting pure states?}

  To embed $\Csr(\G)$ into $\Csr(\tilde \G)$ we first want to embed $C_{\text c}(\G)$ 
  into $C_{\text c}(\tilde \G)$, so we have to show that $Q$ is proper.
  Let $K\subset \G$ be a compact set,
  then the preimage $Q^{-1}(K) = \{ (\gamma, \tilde x) \mid \gamma \in K\}$
  is compact, since $\tilde X$ is.
  %Let $K\subset \G$ be a compact set 
  %and $(\gamma_\lambda, \tilde x_\lambda)$ be a net in $q^{-1}(K)$.
  %Then, as $\gamma_\lambda \in K$, we may pass to a subnet 
  %and assume that $\gamma_\lambda \to \gamma \in K$ in $\G$.
  %As the range map is continuous, $r(K)$ is a compact subset of $X$ 
  %and as $q\colon \tilde X \rightarrow X$ is continuous, 
  %its $q$-preimage is a closed subset of the compact space $\tilde X$, hence compact.
  %Thus, every $\tilde x_\lambda$ is contained in the compact set $q^{-1}\left( r(K) \right)$ 
  %and passing to a subset again we may assume $\tilde x_\lambda \to \tilde x$.
  %This way we found a subnet that converges in $q^{-1}(K)$.

  Since $Q$ is a groupoid homomorphism, 
  precomposition with $Q$ as a map
  $Q^\ast\colon C_{\text c}(\G) \hookrightarrow C_{\text c}(\tilde \G)$ 
  is compatible with the convolution and involution on both algebras.
  We continue by showing that $\|f\|_{\Csr(\G)} = \|f\circ Q\|_{\Csr(\tilde \G)}$
  for $f \in C_c(\G)$,
  so that $Q^\ast$ extends from $C_{\text c}(\G)$ 
  to an embedding of the associated reduced algebras.
  First we notice that $Q$ gives a bijection 
  $\tilde \G_{\tilde x} \rightarrow \G_{q(\tilde x)}$ 
  between the source fibers by $(\gamma, \gamma\tilde x) \mapsto \gamma$.
  Then we obtain an isomorphism 
  $U\colon \ell^{2}(\tilde \G_{\tilde x}) \rightarrow \ell^{2}(\G_{q(\tilde x)})$ 
  by $\delta_{(\gamma, \gamma\tilde x)} \mapsto \delta_\gamma$,
  which intertwines the associated source fiber representations $\pi_{\tilde x}$ and $\pi_x$:
  \begin{align*}
    U \pi_{\tilde x}(f\circ Q) U^{\ast} \,\delta_\gamma
    &= U \pi_{\tilde x}(f\circ Q) \,\delta_{(\gamma, \gamma \tilde x)}\\
    &= U \sum\limits_{\alpha \in \G_x}
    f\circ Q\left( (\alpha, \alpha\tilde x)\right)
    \,\delta_{(\alpha\gamma, \alpha\gamma\tilde x)}\\
    &= U \sum\limits_{\alpha \in \G_{x}}
    f( \alpha ) \,\delta_{(\alpha\gamma, \alpha\gamma\tilde x)}\\
    &= \sum\limits_{\alpha \in \G_{x}} f( \alpha ) \,\delta_{\alpha\gamma}\\
    &= \pi_x(f) \,\delta_\gamma.
  \end{align*}
  Thus the norms of $f$ and $f\circ Q$ coincide 
  and we obtain the desired embedding of $\Csr(\G)$ into $\Csr(\tilde \G)$.
\end{proof}


This embedding is even compatible with ucp extensions in the following sense:
\begin{lemma}
  Let $\pi\colon \Csr(\G) \rightarrow \B(\H)$
  be a $\ast$-representation of $\Csr(\G)$
  whose restriction to $C(X)$ is injective
  and let $\tilde\pi\colon \Csr\left( \tilde \G \right) \rightarrow \B(\H)$
  be a ucp extension of $\pi$.
  Then the $\Cs$-algebra $\intermediaryAlgebra$ 
  generated by $\tilde\pi\left( C\left( \tilde X \right) \right)$
  inside $\B(\H)$
  carries the structure of a $\G$-algebra,
  such that the restriction
  $\tilde\pi|_{C\left( \tilde X \right)} \rightarrow E$ 
  is $\G$-equivariant.
  \label{lem:extendUcpToGAlgebra}
\end{lemma}
\begin{proof}
  Let
  $\intermediaryAlgebra \defeq C^{\ast}\left( \tilde \pi\left( C(\tilde X) \right) \right) 
  \subseteq \B(\H)$ 
  be the $\Cs$-algebra generated in $\B(\H)$
  by the image of $\tilde\pi$ on $C\left( \tilde X \right)$.
  Firstly, as $\tilde \pi$ restricts to $\pi$ on $C(X)$ and is injective there,
  we may identify 
  $C(X) \subseteq \intermediaryAlgebra$ 
  as a subalgebra.
  As $\pi$ is a \starhomomorphism{}, 
  $C\left( X \right)$ lies in the multiplicative domain of $\tilde \pi$, 
  so that this action is central.
  Thus, $\intermediaryAlgebra$ is a $C(X)$-algebra
  and we can consequently define a $\G$-action:
  For $\tilde \pi$ to be $\G$-equivariant, 
  the $\G$-action on 
  $\tilde\pi\left( C\left( \tilde X \right) \right) \subseteq \intermediaryAlgebra$
  obviously has to be
  \[\gamma. \left[ \tilde \pi(f) \right]_x
    = \gamma.\tilde\pi_x\left( \left[ f \right]_x \right)
    \defeq
    \tilde \pi_{\gamma.x}\left( \gamma.\left[ f \right]_x \right)
  \]
  for $f\in C\left( \tilde x \right)$ with $x = s(\gamma)$
  and $\gamma.x = r(\gamma)$.
  Note that if 
  $g_\gamma \in C_c(\G)$ is supported on a bisection of $\G$ 
  and $g_\gamma(\gamma) = 1$,
  then $g_\gamma \ast f \ast g_\gamma^\ast$ is in $C\left( \tilde X \right)$
  and a quick calculation shows that 
  \begin{equation}
    \label{eq:conjugationActionExplicit}
    \left( g_\gamma \ast f \ast g_\gamma^\ast \right)(\tilde x) 
    =
    \left| g_\gamma\left( \left(r|_B \right)^{-1}(\tilde x)\right) \right|^2 
    \cdot f\left(s\circ\left( r|_B \right)^{-1}(\tilde x)\right),
  \end{equation}
  where $B\subseteq \tilde \G$ is the bisection
  on which $g_\gamma\circ q$ is supported.
  Thus $\gamma.[f]_x = \left[ g_\gamma \ast f \ast g_\gamma \right]_{\gamma.x}$
  and since $g_\gamma$ is in the multiplicative domain of $\tilde \pi$
  we can write
  \[
    \gamma. \left[ \tilde\pi(f) \right]_x
    \defeq \tilde\pi_{\gamma.x}\left( \gamma.\left[ f \right]_x \right)
    = \left[ \tilde\pi(g_\gamma) \tilde\pi(f) \tilde\pi(g_\gamma)^\ast \right]_{\gamma.x}.
  \]
  This extends to general $a \in \intermediaryAlgebra$ by
  \begin{equation}
    \gamma. \left[ a \right]_x
    \defeq
    \left[ \tilde\pi(g_\gamma) a \tilde\pi(g_\gamma)^\ast \right]_{\gamma.x}
    \label{eq:actionOnIntermediaryAlgebra}
  \end{equation}
  and we proceed to show that this is a well-defined $\G$-action.
  First we show that $\gamma.[a]_x$ does not depend on the choice of $a$ to represent $[a]_x$.
  By linearity we just have to show that $\gamma.[a]_x = 0$ if $[a]_x=0$,
  that is, if $a \in \overline{C_0\left( X\setminus x \right)\intermediaryAlgebra}$.
  We may thus approximate $a$ by finite sums of elements of the form 
  $h \cdot \tilde\pi(f_1)\cdots\tilde\pi(f_n)$
  with $h \in C_0\left( X\setminus x \right)$
  and $f_i \in C\left( \tilde X \right)$,
  while $n$ varies.
  As the action in Equation \ref{eq:actionOnIntermediaryAlgebra}
  depends continuously on $a$,
  it suffices to show that 
  $\gamma.\left[ h \cdot \tilde\pi(f_1) \cdots \tilde\pi(f_n) \right]_x = 0$.
  As $g_\gamma^\ast \ast g_\gamma$ and $g_\gamma \ast g_\gamma^\ast$
  are supported on $X$
  and $\left[ g_\gamma \ast g_\gamma^\ast \right]_{\gamma.x} = 1$,
  we may now calculate that
  \begin{align*}
    \left[ \pi\left(g_\gamma\right) h \tilde\pi(f_1) 
    \tilde\pi(f_2) \pi\left( g_\gamma \right)^\ast \right]_x
    &=
    \left[ \pi\left( g_\gamma \ast g_\gamma^\ast \right) \right]_{\gamma.x}
    \left[ \pi\left(g_\gamma\right) h \tilde\pi(f_1) 
    \tilde\pi(f_2) \pi\left( g_\gamma \right)^\ast \right]_x
    \\
    &=
    \left[ \pi\left( g_\gamma \ast g_\gamma^\ast \right) 
      \pi\left(g_\gamma\right) h \tilde\pi(f_1) 
    \tilde\pi(f_2) \pi\left( g_\gamma \right)^\ast \right]_x
    \\
    &=
    \left[ \pi\left( g_\gamma \right) 
      \pi\left( g_\gamma^\ast  \ast g_\gamma\right) 
      h \tilde\pi(f_1) 
    \tilde\pi(f_2) \pi\left( g_\gamma \right)^\ast \right]_x
    \\
    &=
    \left[ \pi\left( g_\gamma \right) 
      h \tilde\pi(f_1) 
      \pi\left( g_\gamma\right)^\ast  \pi\left(g_\gamma\right) 
    \tilde\pi(f_2) \pi\left( g_\gamma \right)^\ast \right]_x
    \\
    &=
    \left[ 
      \pi\left( g_\gamma \right) 
      h \tilde\pi(f_1) 
      \pi\left( g_\gamma\right)^\ast
    \right]_{\gamma.x}
    \left[ 
      \pi\left(g_\gamma\right) 
      \tilde\pi(f_2) \pi\left( g_\gamma \right)^\ast 
    \right]_x
    \\
    &=
    \tilde\pi_{\gamma.x}\left( \gamma.\left[ hf_1 \right]_x \right)
    \tilde\pi_{\gamma.x}\left( \gamma.\left[ f_2 \right]_x \right)
    = 0
  \end{align*}
  for $n=2$ and analogously for arbitrary $n$.
  Incidentally, this also shows how the action gives homomorphisms
  between the appropriate fibers, that is,
  \[ \gamma.\left[ a b \right]_x =
    \gamma.\left[ a \right]_x
    \gamma.\left[ b \right]_x.
  \]

  Next we show that $\gamma.\left[ a \right]_x$ is independent 
  of the choice of $g_\gamma$ as above.
  Suppose $g_\gamma$ and $g'_\gamma$ are as described 
  supported on open bisections $B$ and $B'$
  and evaluate to one at $\gamma$.
  As $B\cap B'$ is an open neighborhood of $\gamma$,
  $s\circ \left( r|_B \right)^{-1}$ and
  $s\circ \left( r|_{B'} \right)^{-1}$
  coincide on the neighborhood $r(B\cap B')$ of $r(\gamma)$
  and by Equation \eqref{eq:conjugationActionExplicit}
  we find that
  \[
    \left(g_\gamma \ast f \ast g_\gamma^\ast\right)
    - 
    \left(g'_\gamma \ast f \ast \left( g'_\gamma \right)^{\ast}\right)
    \left( \tilde x \right)
    =
    \underbrace{
      \left( 
        \left| g_\gamma\left( \left( r|_B \right)^{-1}(x) \right) \right|^2
        - 
        \left| g'_\gamma\left( \left( r|_B \right)^{-1}(x) \right) \right|^2
      \right)
    }_{\in C_0\left( X\setminus r(\gamma) \right)}
    \cdot f\left(s\circ\left( r|_B \right)^{-1}(\tilde x)\right).
  \]
  and thus
  \[
    \left[ g_\gamma \ast f \ast g_\gamma^\ast \right]_{r(\gamma)}
    =
    \left[ g'_\gamma \ast f \ast \left( g'_\gamma \right)^\ast \right]_{r(\gamma)}.
  \]
  By approximating arbitrary $a \in \intermediaryAlgebra$
  by finite sums of elements of the form $h\cdot \tilde\pi(f_1) \cdots \tilde \pi(f_n)$
  as above,
  we conclude that the same holds for arbitrary $a$.

  As $\left[ g_\gamma^\ast \ast g_\gamma \right]_x = 1$
  and $g_\gamma^\ast$ is a valid choice for $g_{\gamma^{-1}}$,
  the action of $\gamma$ is invertible by acting with $\gamma^{-1}$.
  Since it furthermore respects conjugation,
  the action is by $\ast$-isomorphisms.
  Furthermore,
  as $g_\eta \ast g_\gamma$ for composable $\eta$ and $\gamma \in \G$
  is supported on a bisection and evaluates to one at $\eta\gamma$,
  it is a valid choice for $g_{\eta\gamma}$.

  Finally, we show that the action is continuous.
  Let $\gamma_\lambda \to \gamma$ 
  and $\left[ a_\lambda \right]_{x_\lambda} \to \left[ a \right]_x$
  with $x_\lambda = s(\gamma_\lambda)$ 
  and $x = s(\gamma)$.
  We have to prove that 
  $\gamma_\lambda.\left[ a_\lambda \right]_{x_\lambda} \to \gamma.\left[ a \right]_x$.
  As the elements of $\intermediaryAlgebra$ 
  are exactly the continuous sections in the associated bundle,
  the convergence $\left[ a_\lambda \right]_{x_\lambda} \to \left[ a \right]_x$
  is equivalent to 
  $\left\| \left[ a_\lambda - a \right]_{x_\lambda} \right\|_{x_\lambda} \to 0$
  and it thus suffices to show that 
  $\gamma_\lambda.\left[ a \right]_{x_\lambda} \to \gamma.\left[ a \right]_x$.
  We do this first for $a = \tilde\pi(f)$ 
  and then generalise to arbitrary $a$ as before.
  As $\tilde\pi$ is $\G$-equivariant we find that
  \[
    \gamma_\lambda.\left[ \tilde\pi(f) \right]_{x_\lambda}
    =
    \tilde\pi_{\gamma_\lambda.x_\lambda}\left( \gamma_\lambda.[ f ]_{x_\lambda} \right)
    \to
    \tilde\pi_{\gamma.x}\left( \gamma.\left[ f \right]_x \right)
    =
    \gamma.\left[ \tilde\pi(f) \right]_{x}.
  \]
  \todocomment{Can also give a longer but more direct proof 
  by calculation instead of using $\tilde\pi$.}

  As the action by $\gamma$ is via a \starhomomorphism{}, the same holds with $\tilde \pi(f)$
  replaced by a linear combination of finite products of this form.
  Since these are dense, convergence 
  $\gamma_\lambda.\left[ a_\lambda\right]_{x_\lambda} \to \gamma.\left[ a \right]_x$
  may be tested against such sections: 
  The net converges to $\gamma.\left[ a \right]_x$, if and only if
  for all $\eps>0,\,  n,k \in \N$, and $ f_{1,1},\ldots, f_{n,k} \in C\left( \tilde X \right)$
  with
  $\|\gamma.[a]_x - [ \sum\nolimits_{i=1}^k\tilde \pi(f_{1,i}) \cdots 
  \tilde \pi(f_{n,i}) ]_{\gamma.x} \|_{\gamma.x} < \eps$
  we eventually have 
  $\| \gamma_\lambda.[ 
  a_\lambda ]_{x_\lambda} 
  - [ \sum\nolimits_{i=1}^k\tilde \pi( f_{1,i} ) \cdots 
    \tilde \pi( f_{n,i} ) 
  ]_{\gamma_\lambda.x_\lambda} \|_{\gamma_\lambda.x_\lambda} 
  < \eps.$

  Let 
  $b = \sum\nolimits_{i=1}^k\tilde\pi\left( f_{1,i} \right) 
  \cdots \tilde\pi\left( f_{n,i} \right)$
  such that $[b]_{\gamma.x}$ approximates $\gamma.[a]_x$ up to $\eps$.
  Then we find that
  \begin{align*}
    \left\|
    \gamma_\lambda.\left[ a \right]_{x_\lambda}
    -
    \left[ b \right]_{\gamma_\lambda.x_\lambda}
    \right\|_{\gamma_\lambda.x_\lambda}
    &=
    \left\|
    \left[ a \right]_{x_\lambda}
    -
    \gamma_\lambda^{-1}.\left[ b \right]_{\gamma_\lambda.x_\lambda}
    \right\|_{x_\lambda}
    \\
    &\leq
    \left\|
    \left[ a \right]_{x_\lambda}
    -
    \left[ 
      \tilde\pi(g_\gamma)^\ast b \tilde\pi(g_\gamma) 
    \right]_{x_\lambda}
    \right\|_{x_\lambda}
    +
    \left\|
    \left[ 
      \tilde\pi(g_\gamma)^\ast b \tilde\pi(g_\gamma) 
    \right]_{x_\lambda}
    -
    \gamma_\lambda^{-1}.\left[ b \right]_{\gamma_\lambda.x_\lambda}
    \right\|_{x_\lambda}
  \end{align*}
  By the arguments above the right-hand term vanishes as $\lambda\to\infty$
  while the left-hand term is the norm of a section and hence
  depends upper semi-continuously on $x_\lambda$.
  Hence
  \[
    \limsup\limits_{\lambda\to \infty}
    \left\|
    \gamma_\lambda.\left[ a \right]_{x_\lambda}
    -
    \left[ b \right]_{\gamma_\lambda.x_\lambda}
    \right\|_{\gamma_\lambda.x_\lambda}
    \leq
    \left\|
    \left[ a \right]_{x}
    -
    \left[ 
      \tilde\pi(g_\gamma)^\ast b \tilde\pi(g_\gamma) 
    \right]_{x}
    \right\|_{x}
    =
    \left\|
    [a]_x
    -
    \gamma^{-1}.\left[ b \right]_{\gamma.x}
    \right\|_x
    <\eps,
  \]
  so the action is continuous.
\end{proof}

\begin{remark}
  Although this method of defining a $\G$-action 
  on the image of a $\G$-algebra under a ucp map as above 
  seems more general than in the given setting,
  we are not aware of it in the literature 
  and are therefore using it ad-hoc as provided.
\end{remark}

\begin{lemma}
  The groupoid $\tilde \G$ has the intersection property
  if $\G$ has the intersection property.
  \label{lem:intersectionPassesToEnvelope}
\end{lemma}
\begin{proof}
  We first prove that the intersection property of $\G$ 
  implies the intersection property of $\tilde \G$.

  Let $\pi\colon \Csr(\tilde \G) \rightarrow A$ be a \starhomomorphism{} 
  with $\ker(\pi)\cap C(\tilde X) = \{0\}$.
  Then $\pi$ restricts to an injective \starhomomorphism{} $\Csr(\G) \rightarrow A$, 
  since $\G$ has the intersection property
  and $\ker(\pi) \cap C(X) \subseteq \ker(\pi) \cap C(\tilde X)$.
  Thus, we may find a ucp map $\psi\colon \pi(\Csr(\G)) \rightarrow C(X)$ 
  such that $\psi \circ \pi|_{\Csr(\G)} = E_X$ 
  is the canonical conditional expectation $E_X\colon \Csr(\G) \rightarrow X$.
  As $\pi$ is injective on $C(\tilde X)$, 
  we may denote the inverse by $\tilde \psi \colon \pi(C(\tilde X)) \rightarrow C(\tilde X)$.
  Then $\tilde \psi$ extends the restriction of $\psi$ to $\pi(C(X))$.
  Thus we obtain a well-defined ucp map 
  from the operator system $\pi(\Csr(\G)) + \pi(C(\tilde X))$ to $C(\tilde X)$
  by $a+b \mapsto \psi(a) + \tilde\psi(b)$ for $a\in \pi\left( \Csr(\G) \right)$ 
  and $b\in \pi\left( C(\tilde X) \right)$.
  \todocomment{Make sure that the sum is indeed an operator system. 
  If necessary, $\Csr(\G) + C(\tilde X)$ is closed in $\Csr(\tilde \G)$.}
  As $C(\tilde X)$ is also an injective operator system, 
  we may extend this map to all of $A$, 
  writing $\phi\colon A \rightarrow C(\tilde X)$
  as in Diagram \eqref{cd:continueToConditionalExpectation}:
  \begin{equation}\label{cd:continueToConditionalExpectation}
    \begin{tikzcd}
      \Csr(\G)
      \ar[r, rightarrow, "\pi"]
      \ar[dd,hookrightarrow]
      & \pi(\Csr(\G))
      \ar[rr, rightarrow, "\psi"]
      \ar[d, hookrightarrow]
      && C(\tilde X)
      \\
      & \pi\left( \Csr(\G) + C(\tilde X) \right)
      \ar[d, hookrightarrow]
      \ar[rru, dashed, "\psi + \tilde \psi"description]
      \\
      \Csr(\tilde \G)
      \ar[r, "\pi"]
      & A
      \ar[rruu, dashed, "\phi"below]
    \end{tikzcd}
  \end{equation}
  Now $\phi \circ \pi \colon \Csr(\tilde \G) \rightarrow C(\tilde X)$ is a ucp map 
  such that
  $(\phi\circ \pi)|_{C(\tilde X)} = \text{id}_{C(\tilde X)}$. 
  Thus $C(\tilde X) \subseteq \mult(\phi\circ \pi)$ 
  and on the dense subset $C_c(\G) \odot C(\tilde X)$ of $\Csr(\tilde \G)$
  we may calculate
  \[
    \phi\circ\pi\left( f \otimes g \right) 
    = \phi\circ\pi(f) \phi\circ\pi(g) 
    = E_X(f) g
    = E_{\tilde X}\left( f\otimes g \right).
  \]
  Thus, $\phi\circ\pi$ coincides with the canonical conditional expectation 
  $E_{\tilde X}\colon \Csr(\tilde \G) \rightarrow C(\tilde X)$.
  As this map is faithful, $\pi$ is faithful and it follows 
  that $\tilde \G$ has the intersection property.
\end{proof}
  \begin{remark}
    It seems remarkable that, contrary to the arguments of Kawabe \cite[Thm. 3.4]{Kawabe}, 
    we did not need to use $\G$-injectivity of $C(\tilde X)$.
  \end{remark}

\begin{lemma}
  The groupoid $\G$ has the intersection property
  if $\tilde \G$ has the intersection property.
  \label{lem:intersectionPassesFromEnvelope}
\end{lemma}
\begin{proof}
  Let $\pi\colon \Csr(\G) \rightarrow \B(\H)$ be a representation 
  of $\Csr(\G)$ with $\ker(\pi) \cap C(X) = \{0\}$.
  By Arveson extension we may find a ucp extension 
  $\tilde \pi\colon \Csr(\tilde \G) \rightarrow \B(H)$
  and we denote by $D = C^\ast\left( \tilde \pi\left( \Csr(\tilde \G) \right) \right)$ 
  the sub-$C^*$-algebra of $\B(\H)$ 
  generated by $\tilde \pi\left( \Csr\left( \G \right) \right)$.
  We consider 
  $\intermediaryAlgebra \defeq C^{\ast}\left( \tilde \pi\left( C(\tilde X) \right) \right) 
  \subseteq D$ 
  as in Lemma \ref{lem:extendUcpToGAlgebra}
  and endow it with the $\G$-algebra structure defined there.

  As $\intermediaryAlgebra$ contains $C(X)$ as a sub-$\G$-algebra, 
  we may find a ucp $\G$-map 
  $\phi\colon \intermediaryAlgebra \rightarrow C\left( \tilde X \right)$
  by extending the inclusion of $C\left( X \right)$.
  Then $\phi \circ \tilde\pi|_{C\left( \tilde X \right)}$ is a $\G$-map 
  fixing $C\left( X \right)$,
  hence by rigidity of $C\left( \tilde X \right)$ it is the identity:
  $\phi \circ \tilde\pi|_{C\left( \tilde X \right)} = \text{id}_{C\left( \tilde X \right)}$.
  Thus, both $\phi|_{\tilde \pi\left( C\left( \tilde X \right) \right)}$ 
  and $\tilde\pi|_{C\left( \tilde X \right)}$ are isometries
  and since 
  $\text{mult}(\phi) 
  = \overline{\text{span}}\left\{ u \bigm| \|u\|=1,\,\phi(u)\text{ unitary} \right\}$,
  $\phi$ is a \starhomomorphism{}, 
  as $\tilde \pi(u)$ for $u \in C\left( \tilde X \right)$ unitary
  belongs to the multiplicative domain of $\phi$
  and these generate $\intermediaryAlgebra$
  as a $\Cs$-algebra.

  However, we cannot conclude that $\tilde \pi|_{C\left( \tilde X \right)}$ 
  is a \starhomomorphism{ }, 
  as $\phi$ might have non-trivial kernel.
  This is alleviated as follows:
  We consider 
  $L= \overline{\ker(\phi) \cdot \tilde\pi\left( C_c\left( \tilde \G \right) \right)} 
  \subseteq D$
  and show that it is an ideal in $D$.
  To this end it is enough to show that 
  $\tilde \pi\left( C_c\left( \tilde \G \right) \right) \ker\left( \phi \right) 
  \subseteq 
  \overline{ \ker\left( \phi \right) \tilde \pi\left( C_c(\tilde \G) \right) }$.
  But first consider $g \in C_c\left( \G \right)$ and $a \in \ker(\phi)$
  and assume $g$ to be real-valued and supported on a bisection $B$.
  \todocomment{The following remark is out of place and should happen earlier:}
  \begin{remark}
    By ``support'' of a function $g$ we
    will refer to the open set $\left\{ x \bigm| g(x) \neq 0 \right\}$,
    not its closure.
    Note that the closure of an open bisection is not necessarily a bisection.
  \end{remark}
  We let $h = \sqrt[3]g$.
  Then $h^\ast \ast h \in C(X)$ is given by 
  \begin{equation*}
    \left( h^\ast \ast h \right)(x) = 
    \begin{cases}
      |h(\gamma_x)|^2 & x \in s(B)\\
      0
    \end{cases}
  \end{equation*}
  where $\gamma_x$ is the unique arrow in $B$ such that $Bx = \{\gamma_x\}$.
  Thus $h\ast h^\ast \ast h = g$
  and $\pi(g)a = \pi\left( h\ast h^\ast \ast h \right) a$.
  Since $h^\ast \ast h \in C(X)$ acts centrally on $\intermediaryAlgebra$,
  we find that 
  $\pi(g)a = \pi(h \ast h^\ast \ast h)a 
  = \left( \pi(h) \cdot a \cdot \pi(h)^\ast \right)\pi(h)$.

  We proceed to argue that $\pi(h) a \pi(h)^\ast \in \ker (\phi)$.
  As $\phi$ is a $\G$-\starhomomorphism{ },
  this amounts to showing that 
  $\left[ \pi(h)a\pi(h)^\ast \right]_x \in \ker\left( \phi_x \right)$
  for all $x\in X$.
  First assume $x \not \in r(B)$.
  Then let $k = \sqrt[3] h$ and note that $k^\ast \ast k \in C_0\left( X\setminus x \right)$.
  Thus
  \begin{equation*}
    \left[ \pi(h) a \pi(h)^\ast \right]_x
    = 
    \left[ \pi(kk^\ast) \pi(k) a \pi(h)^\ast \right]_x
    =
    \left[ \pi(kk^\ast)\right]_x \left[ \pi(k) a \pi(h)^\ast \right]_x
    = 
    0.
  \end{equation*}
  On the other hand, if $x \in r(B)$ with $xB = {\gamma}$,
  we may rescale $h$ by $1/h(\gamma)$ to $h' = h/h(\gamma)$.
  Then by definition of the $\G$-action 
  \begin{equation*}
    h(\gamma)^2 \cdot \gamma.\left[ a \right]_{s(\gamma)}
    =
    h(\gamma)^2 \left[ \pi(h') a \pi(h')^\ast \right]_x
    = 
    \left[ \pi(h) a \pi(h)^\ast \right]_x.
  \end{equation*}
  Now since $\phi$ is a $\G$-map,
  $\gamma.[a]_{s(\gamma)}$ is in the kernel of $\phi_x$
  exactly if $[a]_{s(\gamma)}$ is in the kernel of $\phi_{s(\gamma)}$,
  which holds if $a\in \ker(\phi)$.
  Thus, for $g\in C_c(\G)$ real-valued and supported on a bisection
  we find that
  \begin{equation*}
    \pi(g) a =
    \left( \pi(h)\cdot a \cdot \pi(h)^\ast \right) 
    \pi(h) \in \ker(\phi) \cdot \pi\left( C_c\left( \G \right) \right)
  \end{equation*}
  and as such $g$ span $C_c(\G)$ densely
  we may conclude that 
  $\pi\left( C_c\left( \G \right) \right) \ker(\phi) 
  \subseteq \overline{\ker(\phi) \pi\left( C_c\left( \G \right) \right)}$.
  To handle more general $g\in C_c\left( \tilde \G \right)$,
  we note that $C_c\left( \G \right) \cdot C\left( \tilde X \right)$ 
  spans $C_c\left( \tilde \G \right)$ densely
  and that $C\left( \tilde X \right)\ker\left( \phi \right) \subseteq \ker\left( \phi \right)$,
  so that the examples above span a dense subset of 
  $\tilde \pi\left( C_c\left( \tilde \G \right) \right)\ker\left( \phi \right)$.
  Thus $L$ is an ideal of $D$
  whose elements are exactly these fixed by left multiplication with an approximate unit 
  of $\ker(\phi) \subseteq \intermediaryAlgebra$.
  Hence $L\cap \intermediaryAlgebra = \ker(\phi)$.

  Denoting by $\Phi$ the quotient map $D \rightarrow D/L$,
  we consider the ucp map $\Phi \circ \tilde \pi$.
  As $\phi$ naturally factors through the restriction of $\Phi$ to $\intermediaryAlgebra$,
  and $\phi \circ \left( \Phi \circ \tilde \pi \right)|_{C\left( \tilde X \right)} 
  = \text{id}_{C\left( \tilde X \right)}$
  we may now conclude that 
  $\left( \Phi \circ \tilde \pi \right)|_{C\left( \tilde X \right)}$ 
  is a \starhomomorphism{ }
  since $\phi$ is an injective left inverse on $\intermediaryAlgebra / L \subseteq D/L$.
  Additionally, $\left( \Phi \circ \tilde \pi \right)|_{\Csr\left( \G \right)} = \Phi \circ \pi$
  is a \starhomomorphism{ },
  so both $C\left( \tilde X \right)$ and $\Csr\left( \G \right)$
  belong to the multiplicative domain of $\Phi \circ \tilde \pi$.
  As their product is dense in $\Csr\left( \tilde \G \right)$
  it follows that $\Phi \circ \tilde \pi$ itself is a \starhomomorphism{}.
  However, $\Phi \circ \tilde \pi$ is faithful on $C\left( \tilde X \right)$
  since 
  $\phi \circ \left( \Phi \circ \tilde \pi \right)|_{C\left( \tilde X \right)} 
  = \text{id}_{C\left( \tilde X \right)}$,
  and thus by the intersection property of $\tilde \G$,
  it is itself faithful.
  As $\tilde \pi$ extends $\pi$,
  we may conclude that $\pi$ is faithful on $\Csr\left( \G \right)$.
  Thus $\G$ has the intersection property.
\end{proof}

Having recast the problem of determining whether $\G$ has the intersection property
as answering the same question for $\tilde \G$,
we explore the properties making $\tilde \G$ more tractable:
\begin{lemma}
  All stabiliser groups of $\tilde \G$ are amenable.
  \label{lem:amenableStabilisers}
\end{lemma}
\begin{proof}
  As the $\G$-algebra $l^{\infty}\left( \G \right)$ contains $C(X)$,
  there is a $\G$-equivariant map 
  $\phi\colon l^\infty\left( \G \right) \rightarrow C\left( \tilde X \right)$.
  Then $\text{ev}_{\tilde x} \circ \phi$ provides a state on $l^\infty\left( \G \right)$ 
  that is invariant under the action 
  of the subgroup $\text{Stab}(\tilde x)$ of $G_{q(x)}^{q(x)}$.
  By embedding $l^\infty\left( \text{Stab}(\tilde x) \right)$ into $l^\infty\left( \G \right)$
  we obtain an invariant state on 
  $l^\infty\left( \text{Stab}(\tilde x) \right) 
  = l^{\infty}\left( \tilde \G_{\tilde x}^{\tilde x} \right)$.
\end{proof}

\begin{lemma}
  Let $Z\subseteq \tilde X$ be a closed $\G$-invariant subset such that $q(Z) = X$. 
  Then $Z = \tilde X$.
  \label{lem:equivariance}
\end{lemma}
\begin{proof}
  As $q$ restricted to $Z$ is still surjective, we can embed $C(X)$ into $C(Z)$ 
  and, by $\G$-injectivity of $C(\tilde X)$,
  extend the embedding $C(X) \hookrightarrow C(\tilde X)$ 
  to a ucp map $\phi\colon C(Z) \rightarrow C(\tilde X)$.
  Then the composition
  with restriction to $Z$ 
  \[ C(\tilde X) \xrightarrow{\text{res}_Z} C(Z) \xrightarrow \phi C(\tilde X) \]
  is a $\G$-equivariant ucp map $C(\tilde X) \rightarrow C(\tilde X)$ 
  that restricts to the identity on the subalgebra $C(X)$.
  By rigidity of the $\G$-equivariant injective envelope, 
  it is therefore the identity on all of $C(\tilde X)$.
  Thus, $\text{res}_Z$ is injective, hence $Z$ is dense. 
  As it is also closed, we get $Z=\tilde X$.
\end{proof}

\begin{lemma}
  If every orbit of $\tilde \G$ has at least two points,
  then the isotropy bundle $\text{Iso}\left( \tilde \G \right)$ of $\tilde \G$ is clopen.
  \label{lem:clopenIsotropy}
\end{lemma}
If $\G$ already has orbits consisting of at least two points, 
then so does $\tilde \G$.
In particular this is the case when $\G$ is minimal,
so it bears no restriction in investigating simplicity of reduced groupoid algebras.
We are of course tacitly avoiding the case where $\G$ is a group
so that orbits cannot consist of two distinct points
because $\G^{\left( 0 \right)}$ is a single point.
\begin{proof}
  For every groupoid the isotropy bundle is closed, so we have to show that it is open.
  Consider $\gamma \in \tilde \G_{\tilde x}^{\tilde x}$.
  As $C(\tilde X)$ is an injective algebra, $\tilde X$ is Stonean
  and in particular zero-dimensional.
  Thus there exists a \textit{full} open bisection $B$ containing $\gamma$,
  that is,
  a open bisection with $s(B) = \tilde X = r(B)$
  by \sourcecomment{Kevin's Paper \cite{Kevin}}.
  Then $B$ defines a homeomorphism $\tilde X \rightarrow \tilde X$
  by $r\circ (s|_{B'})^{-1}$
  whose fixed point set $F$ contains $s(\gamma) = \tilde x = r(\gamma)$.
  By Frolik's theorem \sourcecomment{\cite{Frolik}}
  this fixed point set is open
  and thus $B \cap s^{-1}(F)$ is an open neighborhood of $\gamma$
  contained in the isotropy.
\end{proof}
\begin{remark}
  This of course works in general for every groupoid with Stonean unit space
  and orbits consisting of at least two points.
  Until now we failed to drop this second condition, 
  although it holds true for the case of crossed products by groups.
  In particular, it is not necessary for every $\gamma$ to be contained
  in a full bisection,
  even with the current proof it suffices to be contained in an open bisection $B$
  which has full source $s(B) = \tilde X$.
\end{remark}

These already enable us to prove one implication of our main theorem:
\begin{theorem}
  If $\G$ satisfies the condition of Proposition \ref{thm:main} 
  then it has the intersection property.
  \label{thm:conditionSufficient}
\end{theorem}
\begin{proof}
  Let as before $q$ denote the continuous map $\tilde \G \rightarrow \G$
  given by $\left( \tilde x, \gamma \right) \mapsto \gamma$.
  Let $\Lambda = \left\{ q(\text{Stab}(\tilde x)) \mid \tilde x \in \tilde X \right\}$.
  By Lemma \ref{lem:amenableStabilisers}, 
  $q(\text{Stab}(\tilde x))$ is an amenable subgroup of $\G_{q(x)}^{q(x)}$,
  so we can conclude that 
  $\overline{\G.\Lambda}\supseteq \left\{ \left\{ x \right\} \bigm | x \in X \right\}$.
  However, $\Lambda$ is already invariant since
  $\gamma.\text{Stab}(\tilde x) 
  = \gamma \text{Stab}(\tilde x)\gamma^{-1} 
  = \text{Stab}(\gamma.\tilde x)$
  and is furthermore closed:
  Let $\Phi\colon \tilde X \rightarrow \text{Sub}\left( \G \right)$
  be the stabiliser map 
  $\tilde x \mapsto q\left(\text{Stab}(\tilde x)\right)$.
  Then $\Lambda$ is the range of $\Phi$ 
  and since $\tilde X$ is compact and $\text{Sub}(\G)$ Hausdorff,
  $\Lambda$ is closed provided that $\Phi$ is continuous.

  Recall that a basis of the topology of $\text{Sub}(\G)$
  is given by the collections
  \begin{align*}
    \O_U &= \left\{ Y \subset \G \bigm| Y \cap U \neq \emptyset \right\}
    &&\text{and}&
    \O'_K &= \left\{ Y \subseteq \G \bigm| Y \cap K = \emptyset \right\}
    \intertext{
      for $U\subseteq \G$ open
      and $K\subseteq \G$ compact.
      We thus calculate
    }
    \Phi^{-1}\left( \O_U \right)
    &= \left\{ 
      \tilde x \bigm| \tilde \G_{\tilde x}^{\tilde x} \cap Q^{-1}(U) \neq \emptyset 
    \right\}
    &&\text{and}&
    \Phi^{-1}\left( \O'_K \right)
    &= \left\{ 
      \tilde x \bigm| \tilde \G_{\tilde x}^{\tilde x}\cap Q^{-1}(K) = \emptyset 
    \right\}\\
    &= s\left( \text{Iso}\left( \tilde \G \right) \cap Q^{-1}\left( U \right) \right)
    &&&
    &= \tilde X \setminus s\left( \text{Iso}\left( \tilde \G \right) \cap Q^{-1}(K) \right).
  \end{align*}
  Since $\tilde X$ is Stonean, $\text{Iso}\left( \tilde \G \right)$ is clopen
  by Lemma \ref{lem:clopenIsotropy},
  and furthermore $s$ is an open map
  while $Q^{-1}(U)$ and $Q^{-1}(K)$ are open and closed, respectively.
  Thus, $\Phi$ is continuous
  and $\Lambda = \Phi\left( \tilde X \right)$ is closed.
  Now $\Lambda \supseteq \left\{ \left\{ x \right\} \bigm | x \in X \right\}$,
  so for all $x \in X$ there is $\tilde x \in \tilde X$
  with $\tilde G_{\tilde x}^{\tilde x} = \left\{ \tilde x \right\}$,
  that is, there are enough trivial isotropies in $\tilde \G$
  to cover $X$ along $q$.
  Hence $Z = \left\{ \tilde x \in \tilde X \bigm| \tilde \G_{\tilde x}^{\tilde x} \right\}$
  is a $\G$-invariant subset of $\tilde X$ with $q(Z) = X$.
  Furthermore $Z$ is closed, 
  since it's complement
  $\tilde X \setminus Z = s\left( \text{Iso}\left( \tilde \G \setminus \tilde X \right) \right)$
  is the image of a closed set under the open, surjective map $s$.
  Thus $Z = \tilde X$ by Lemma \ref{lem:equivariance}, so $\tilde \G$ is principal
  and hence has the intersection property.
  By Lemma \ref{lem:iffIntersection}, the groupoid $\G$ also has the intersection property.
\end{proof}

To obtain the converse implication, 
we establish some further useful properties of $\tilde \G$
if it has the intersection property:

\begin{lemma}
  Restriction to the isotropy subgroupoid $\text{Iso}\left( \tilde \G \right)$
  of $\tilde \G$ is a generalized conditional expectation.
  \label{lem:isotropyExpectation}
\end{lemma}
We use the definition of generalized conditional expectation from 
\cite[Appendix D]{Paterson}, 
where it is described how continuous representations
can be induced from the range of such expectations to their domain,
as is our intention.
\begin{proof}
  List of conditions:
  \begin{itemize}
    \item $A,B$ pre-$C^\ast$-algebras, $B$ acting on $A$ by right multipliers,
      action jointly norm-continuous
    \item $P(a.b) = P(a)b$ (easy)
    \item $a\mapsto P(c^\ast a c)$ is bounded
    \item $\forall a, \eps>0 \, \exists c \in \text{span}(A\cdot A)\colon \| P\left( (a-c)^\ast (a-c) \right)\| < \eps$
    \item P(A) generates a dense subalgebra of $B$ (easy)
    \item $P$ is positive
    \item $P$ is linear, self-adjoint (easy)
  \end{itemize}
  \todocomment{To be done.}
\end{proof}

We consider the orbit equivalence relation groupoid 
$\tilde \G / \text{Iso}(\tilde \G)$ of $\tilde \G$.
Its source fibers $\tilde \G_{\tilde x} / \tilde \G_{\tilde x}^{\tilde x}$ at $\tilde x$
is via the range map 
in canonical bijection with the orbit $r\left( \tilde \G_{\tilde x} \right)$
of $\tilde x$,
so we will write its elements as $(\tilde y, \tilde x)$
to represent the class of $\tilde \G_{\tilde x}^{\tilde y}$.
Now consider the representation $\pi$
of $\Csr(\tilde \G)$
on $\H_\pi = l^2\left( \tilde \G / \text{Iso}(\tilde \G) \right)$
by
\begin{equation*}
  \pi(f)\delta_{(\tilde y, \tilde x)} 
  = \sum\limits_{\gamma \in \tilde \G_{\tilde y}}f(\gamma) \delta_{(r(\gamma), \tilde x)}.
\end{equation*}
By fixing $\tilde x$ we can write
$\pi = \bigoplus_{\tilde x \in \tilde X} \pi_{\tilde x}$
with $\pi_{\tilde x}$
the representation on the invariant subspace 
$l^{2}\left( \tilde \G_{\tilde x} / \tilde \G_{\tilde x}^{\tilde x} \right)$.

\begin{lemma}
  The representation $\pi$ defined above is continuous.
  \label{lem:principalRepresentationContinuous}
\end{lemma}
\begin{proof}
  The isotropy subgroupoid $\text{Iso}\left( \tilde \G \right)$ is just a group bundle
  consisting of the stabilizer groups which are all amenable.
  Hence the trivial representation $\tau$ of $\text{Iso}\left( \tilde \G \right)$ is continuous.
  Explicitly, it is given by
  \[
    \tau(f) \delta_{\tilde x} = 
    \left(
      \sum\limits_{\gamma \in \tilde \G_{\tilde x}^{\tilde x}}f(\gamma) 
    \right) \delta_{\tilde x}
    \qquad \text{on} \qquad
    \H = l^2\left( \tilde X \right)
  \]
  where $f \in C_c\left( \text{Iso}\left( \tilde \G \right) \right)$
  and $\delta_{\tilde x} \in \H$ the indicator at $\tilde x$.
  As in $\cite[Appendix D]{Paterson}$, 
  $\H$ is a left $C_c\left( \text{Iso}\left( \tilde \G \right) \right)$-module via $\tau$
  and $C_c(\tilde \G)$ is a 
  $C_c\left( \tild \G \right)$-$C_c\left( \text{Iso}\left( \tilde \G \right) \right)$ bimodule,
  and we form the induced Hilbert space $\text{Ind}\H$ by completing the balanced tensor product
  $C_c(\tilde \G) \otimes_{C_c\left( \text{Iso}\left( \tilde \G \right) \right)} \H$
  with respect to the (non-definite) inner product given by
  \[
    \left\langle f' \ast \delta', f\ast \delta \right\rangle
    \defeq
    \left\langle 
    \tau\left( P\left( f^\ast \ast f' \right) \delta' , \delta\right) 
    \right\rangle_\H
  \]
  on elementary tensors.
  %, with $mu$ the quasi-invariant measure of $\tau$.
  Thus we may calculate for $f$ and $\delta_{\tilde x}$ as above:
  \begin{align*}
    \left\| f\otimes \delta_{\tilde x} \right\|^2
    =
    \left| 
    \sum\limits_{\eta \in \tilde \G_{\tilde x}^{\tilde x}} f^\ast \ast f(\eta) 
    \right|
  \end{align*}
  Writing $\bar\alpha \in \tilde \G_{\tilde x} / \tilde \G_{\tilde x}^{\tilde x}$
  for the equivalence class $\alpha \tilde \G_{\tilde x}^{\tilde x}$
  of $\alpha \in \tilde \G_{\tilde x}$, we furthermore find that
  \begin{align*}
    \sum\limits_{\eta \in \tilde \G_{\tilde x}^{\tilde x}}(f^{\ast}\ast f)(\eta)
    &=
    \sum\limits_{\eta \in \tilde \G_{\tilde x}^{\tilde x}}
    \sum\limits_{\alpha \in \tilde \G_{\tilde x}} \bar f(\alpha) f(\alpha\eta)
    \\
    &=
    \sum\limits_{\bar\alpha \in \tilde \G_{\tilde x} / \tilde G_{\tilde x}^{\tilde x}}
    \sum\limits_{\eta' \in \tilde G_{\tilde x}^{\tilde x}}
    \left( 
      \bar f(\alpha \eta')
      \sum\limits_{\eta\in \G_{\tilde x}^{\tilde x}}
      f(\alpha \eta' \eta)
    \right)
    \\
    &=
    \sum\limits_{\bar\alpha \in \tilde \G_{\tilde x} / \tilde G_{\tilde x}^{\tilde x}}
    \left |
    \sum\limits_{\eta\in \tilde \G_{\tilde x}^{\tilde x}} f(\alpha \eta)
    \right |^{2}.
  \end{align*}
  And thus for $\xi = \sum \xi_{\tilde x} \delta_{\tilde x} \in \H$ we find that
  \[
  \| f \otimes \xi \|^2
  =
  \sum\limits_{\bar\alpha \in \tilde \G_{\tilde x} / \tilde G_{\tilde x}^{\tilde x}}
  \left(\left|
    \sum\limits_{\alpha \in \bar\alpha} f(\alpha) 
    \xi_{\tilde x}
  \right|^2 \right),
  \]
  and the induced Hilbert space $\text{Ind} \H$
  is isomorphic to $\H_\pi$
  via the isomorphism given by
  \[
    f \otimes \delta_{\tilde x} \mapsto 
    \left( \bar\alpha \mapsto 
    \sum\limits_{\alpha\in\bar\alpha} f(\alpha) \right)
    \in l^2\left( \tilde \G_{\tilde x} / \tilde \G_{\tilde x}^{\tilde x} \right).
  \]

  Under this isomorphism, the preimage of $\delta_(\tilde y,\tilde x) \in \H_\pi$ as above
  is represented by $f\otimes \delta_{\tilde x}$ for $f$ supported on a bisection 
  and with $f(\alpha) = 1$ for some $\alpha$ with source and range $\tilde x$ and $\tilde y$.
  Then for any $g \in C_c(\tilde G)$ the induced representation $\text{Ind} \tau$
  acts as
  \begin{align*}
    \text{Ind}\tau(g) (f\otimes \delta_{\tilde x})
    &= (g\ast f) \otimes \delta_{\tilde x},
    \intertext{which under the isomorphism is identified with}
    &= \sum\limits_{\eta\in \tilde \G_{\tilde x}}(g\ast f)(\eta) \delta_{(r(\eta), \tilde x)}.
    \intertext{
      A quick calculation shows that for $\eta \in \tilde \G_{\tilde x}$ we have
      $(g\ast f)(\eta) = g(\eta\alpha^{-1})$
      and therefore
    }
    &= \sum\limits_{\eta \in \tilde \G_{\tilde x}} g(\eta \alpha^{-1}) 
    \delta_{(r(\eta), \tilde x)}\\
    &= \sum\limits_{\gamma \in \tilde \G_{\tilde x}} g(\gamma ) 
    \delta_{(r(\gamma), \tilde x)}\\
    &= \pi(g) \delta_{(\tilde y, \tilde x)}.
  \end{align*}
  So $\pi$ is nothing else than the induced representation of $\tau$
  and therefore continuous.
\end{proof}

\begin{lemma}
  If $\tilde \G$ has the intersection property, 
  then it is principal.
  \label{lem:intersectionImpliesPrincipal}
\end{lemma}
\begin{proof}
  We use the continuous representation $\pi$ from above.
  If $f\in C\left( \tilde X \right)$, then 
  \begin{equation*}
    \pi(f)\delta_{(\tilde y, \tilde x)} 
    = f\left( \tilde y \right) \delta_{(\tilde y, \tilde x)},
  \end{equation*}
  so $\pi|_{C\left( \tilde X \right)}$ is faithful.
  Thus $\pi$ itself is faithful, 
  if $\tilde \G$ has the intersection property.

  This, however, implies that $\tilde \G$ is principal:
  Were it not, then we could find an open bisection $B$
  contained in the clopen set $\text{Iso}\left( \tilde \G \right) \setminus \tilde X$
  and we could find a nonzero continuous function $f$ supported on $B$.
  Then consider $f' \in C\left( \tilde X \right)$ given by
  $f' = f \circ \left( r|_B \right)^{-1}$ on $r(B)$ and zero outside.
  We may calculate
  \begin{align*}
    \pi\left( f - f' \right)\delta_{(\tilde y, \tilde x)}
    &= \sum\limits_{\gamma \in \tilde \G_{\tilde y}} 
    \left( f(\gamma) - f'(\gamma) \right) \delta_{(r(\gamma), \tilde x)}\\
    &= \left[ \sum\limits_{\gamma \in \tilde \G_{\tilde y}^{\tilde y}}
      f(\gamma) \delta_{(\tilde y, \tilde x)} 
    \right]
    - f'\left( \tilde y \right)\delta_{(\tilde y, \tilde x)}
    \\
    &=
    f\left( \left( r|_B \right)^{-1}(\tilde y) \right) \delta_{(\tilde y, \tilde x)}
    -
    f\left( \left( r|_B \right)^{-1}(\tilde y) \right) \delta_{(\tilde y, \tilde x)}
    \\
    &= 0
  \end{align*}
  which contradicts the faithfulness of $\pi$,
  as $f-f' \neq 0$.
\end{proof}

\begin{lemma}
  If $\G$ has the intersection property,
  then the only ucp map $\phi\colon \Csr\left( \G \right) \rightarrow C(\tilde X)$
  that fixes $C(X)$ pointwise
  is the canonical conditional expectation of $\Csr\left( \G \right)$.
  \label{lem:uniqueExpectation}
\end{lemma}
\begin{proof}
  Let $\phi$ be as described.
  Consider the operator system 
  $O \defeq \Csr\left( \G \right) + C\left( \tilde X \right)$
  inside $\Csr\left( \tilde \G \right)$.
  We may lift $\phi$ to a ucp map 
  $\phi + \text{id}\colon O \rightarrow C\left( \tilde X \right)$
  by 
  \begin{equation*}
    (\phi + \text{id})( a + f) = \phi(a) + f.
  \end{equation*}
As $\phi$ is the identity on $C\left( X) \right)$, this is well-defined.
Then, by injectivity of $C\left( \tilde X \right)$,
we may lift to a ucp map 
$\tilde \phi\colon \Csr\left( \tilde \G \right) \rightarrow C\left( \tilde X \right)$
which restricts to the identity on $C\left( \tilde X \right)$, since $\phi + \text{id}$ did.
\todocomment{It seems suspicious that we use injectivity
  but not $\G$-injectivity of $C\left( \tilde X \right)$.
Is the intermediary lift really ucp?}

Thus, $\tilde \phi$ is a conditional expectation,
as it is an idempotent ucp map.
If $\G$ has the intersection property,
then so does $\tilde \G$ by Lemma \ref{lem:iffIntersection}
and is therefore principal by Lemma \ref{lem:intersectionImpliesPrincipal}.
As the canonical conditional expectation is unique on a principal groupoid
\sourcecomment{\cite[Thm 5.1.13]{SimsNotes}},
$\tilde \phi$ is the canonical expectation.
Hence so is its restriction $\phi$.
\end{proof}

\begin{theorem}
  If $\G$ has the intersection property,
  then it satisfies the condition of Proposition \ref{thm:main}.
  \label{thm:conditionNecessary}
\end{theorem}
\begin{proof}
  Let $\Lambda$ as in Proposition \ref{thm:main}.
  We may assume that $\Lambda$ is compact and $\G$-invariant
  by replacing it with the orbit closure $\overline{\G.\Lambda}$.
  Denoting by $p\colon \Lambda \rightarrow X$ the map 
  that sends a subgroup of $\G_x^{x}$ to $x$,
  we may embed $C(X)$ into $C(\Lambda)$ along $p$.
  This makes $C(\Lambda)$ a $C(X)$-algebra
  with fiber $C\left(p^{-1}(x)\right)$ at $x$.
  As $\G$ acts on the argument via 
  $\gamma.\Lambda_x = \gamma \Lambda_x \gamma^{-1}$
  for $\Lambda_x \in p^{-1}\left( s\left( \gamma \right) \right)$,
  it is even a $\G$-algebra.
  Hence we can extend the embedding of $C\left( X \right)$
  in $C\left( \tilde X \right)$
  to a $\G$-equivariant ucp map 
  $\mu \colon C\left( \Lambda \right) \rightarrow C\left( \tilde X \right)$
  by $\G$-injectivity.

  Consider the map $\theta\colon C_c\left( \G \right) \rightarrow C\left( \Lambda \right)$
  given by 
  \begin{equation*}
    \theta(f)\left( \Lambda_x \right) 
    = \sum\limits_{\gamma \in \Lambda_x}f(\gamma).
  \end{equation*}
  Indeed, $\theta(f)$ is a continuous function:
  Let $\Lambda_x \in \Lambda$
  and $\Lambda_{x_i}\to \Lambda_{x}$ be a convergent net in $\Lambda$. 
  As $X$ is open in $\G$, it follows in particular that $x_i\to x$ in $X$.
  As the support of $f$ is compact, 
  the set $\supp(f)\cap \Lambda_x \eqcolon K = \{t_1\ldots t_n\}$ is finite 
  and for each $t_j$ we may choose an open neighborhood $V_j$ of $t_j$, 
  on which $\|f - f(t_j)\|_\infty < \eps$.
  As $\G$ is \etale, the source map is a local homeomorphism 
  and we may choose the neighborhoods 
  such that it restricts to a homeomorphism on each.
  Furthermore consider the compact set 
  \begin{equation*}
    V_\infty \defeq \supp(f)\setminus\left(\bigcup\limits_{j=1}^n V_j\right)
  \end{equation*}
  which has empty intersection with $\Lambda_x$.
  Thus, $\O'_{V_\infty}$ is a neighborhood of $\Lambda_x$ 
  and for 
  $\Lambda_{x_i} \in \bigcap\limits_{j\in \{1\ldots n\}} \O_{V_j} \cap \O'_{V_\infty}$
  we find that
  \begin{align*}
    \theta(f)(\Lambda_{x_i}) 
    =
    \sum\limits_{j=1}^n \sum\limits_{t\in V_j\cap \Lambda_{x_i}} f(t).
  \end{align*}
  Observe that $V_j$ intersects $\Lambda_{x_i}$
  in exactly one point,
  say $V_j \cap \Lambda_{x_i} = \{t'_j\}$, 
  with $|f(t_j) - f(t'_j)|<\eps$.
  Hence
  \begin{align*}
    |\theta(f)(\Lambda_x) - \theta(f)(\Lambda_{x_i})|
    =
    \left| \sum\limits_{j=1}^n f(t_j) - \sum\limits_{j=1}^n f(t'_j)\right| 
    \leq n \cdot \eps.
  \end{align*}
  Thus $\theta(f)$ is continuous.
  Furthermore $\theta$ is positive,
  that is $\theta\left( f^\ast f \right)(\Lambda_x) \geq 0$
  for all $f\in C_c\left( \G \right)$ and $\Lambda_x \in \Lambda$:
  \begin{align*}
    \theta\left( f^\ast f \right)\left( \Lambda_x \right)
    &=\sum\limits_{t\in \Lambda_x} f^\ast \ast f(t)
    = \sum\limits_{t\in \Lambda_x}\sum\limits_{\gamma\in\G_x}\bar f(\gamma)f(\gamma t)
    \\
    &=\sum\limits_{\gamma\in\G_x}\left( 
      \bar f(\gamma) \sum\limits_{t\in \Lambda_x} f(\gamma t)
    \right).
    \intertext{
      Consider the quotient $\G_x/\Lambda_x$ 
      by the equivalence relation 
      $\gamma \sim \eta \Leftrightarrow \gamma^{-1}\eta \in \Lambda_x$.
      Then
    }
    \theta\left( f^\ast f \right)\left( \Lambda_x \right)
    &=\sum\limits_{[\gamma] \in \G_x/\Lambda_x}
    \sum\limits_{t' \in \Lambda_x} 
    \left(
      \bar f(\gamma t')
      \sum\limits_{t\in \Lambda_x} f(\gamma t' t)
    \right)\\
    &=\sum\limits_{[\gamma] \in \G_x/\Lambda_x}\left(
      \left( \sum\limits_{t' \in \Lambda_x} 
        \bar f(\gamma t')
      \right) \left(
        \sum\limits_{t\in \Lambda_x} f(\gamma t)
      \right)
    \right)\\
    &=\sum\limits_{[\gamma] \in \G_x/\Lambda_x}
    \left| \sum\limits_{t \in \Lambda_x} \bar f(\gamma t) \right|^{2}
    \geq 0.
  \end{align*}

  To extend $\theta$ to a bounded linear map $\Csr\left( \G \right) \rightarrow C(\Lambda)$
  it is crucial that the subgroups in $\Lambda$ are amenable:
  We have to show that $\theta \colon C_c\left( \G \right) \rightarrow C\left( \Lambda \right)$
  is bounded in the norm of $\Csr\left( \G \right)$.
  Equivalently, $\left| \sum\limits_{t\in \Lambda_x} f(t) \right| \leq \| f \|_{\Csr(\G)}$
  for every $\Lambda_x \in \Lambda$.
  Fix $x\in X$. 
  Then the restriction $\Csr(\G) \rightarrow \Csr\left( \G_x^x \right)$
  sending $f\in C_c(\G)$ to $\sum\limits_{t \in \G_x^x} f(t) \lambda_t$
  is bounded, since
  \[ 
    \lambda\left( f|_{\G_x^x} \right) = P\pi_x(f)P^\ast
  \]
  for $\lambda$ the regular representation of the group $\G_x^x$,
  $\pi_x$ the regular representation of $\G$ on $\B(l^2(\G_x))$
  and $P\colon l^2(\G_x^x) \hookrightarrow l^2(\G_x^x)$ the embedding as a subspace.
  Since $\Lambda_x\subseteq \G_x^x$ is a subgroup, 
  there is a canonical conditional expectation $\Csr(\G_x^x) \rightarrow \Csr(\Lambda_x)$
  and since $\Lambda_x$ is amenable, the trivial representation extends to $\Csr(\Lambda_x)$.
  Thus, the map
  \begin{align*}
    \Csr(\G) &\rightarrow \Csr\left( \G_x^x \right)
    \rightarrow \Csr\left( \Lambda_x \right)
    \rightarrow \Cpx\\
    \text{by}\qquad
    f &\mapsto \sum\limits_{t\in \G_x^x} f(t)\lambda_t
    \mapsto \sum\limits_{t\in \Lambda_x} f(t)\lambda_t
    \mapsto \sum\limits_{t\in \Lambda_x} f(t)
  \end{align*}
  is bounded as the composition of bounded maps.

  Since every positive element of $\Csr\left( \G \right)$ is of the form $a^\ast a$
  and we may approximate $a$ in $C_c\left( \G \right)$,
  the extension is still a positive, unital map
  and thus ucp, as the codomain is commutative.
  \todocomment{Instead of this positivity argument, 
    one could redo the previous positivity proof 
    for the map $\Csr(\G) \rightarrow \Csr(\G_x^x)$
  which is replaces the corresponding conditional expectation for crossed products.}

  As $\theta(h) = h \circ p$ for $h\in C(X)$,
  the composition 
  \begin{equation*}
    \Csr(\G)
    \xrightarrow{\theta}
    C\left( \Lambda \right)
    \xrightarrow{\mu}
    C\left( \tilde X \right)
  \end{equation*}
  is a ucp map $\Csr\left( \G \right) \rightarrow C\left( \tilde X \right)$
  fixing $C\left( X \right)$, 
  where $\mu$ is the map defined above 
  by extending from the inclusion $C\left( X \right) \hookrightarrow X$.
  By Lemma \ref{lem:uniqueExpectation}
  it therefore coincides with the canonical conditional expectation
  on $\Csr\left( \G \right)$.
  From here on we may repeat the final part in the proof of
  \cite[Thm 5.2]{Kawabe},
  although in a somewhat more streamlined format.
  Take any $x\in X$
  and any $\tilde x \in \tilde X$ with $q\left( \tilde x \right) = x$
  and consider $\text{ev}_{\tilde x}\circ \mu$.
  Note that $\text{ev}_{\tilde x}\circ \mu(f) = 0$
  if $f$ vanishes on $p^{-1}(x)$:
  For every $\eps >0$ we may pick a neighborhood $U$ of $x$ in $X$
  such that $f$ is bounded by $\eps$ on $p^{-1}\left( U \right)$
  and find $h \in C(X)$ with $0\leq h\leq 1$ and $h(x)=1$.
  Then
  \begin{equation*}
    \left| \text{ev}_{\tilde x} \circ \mu (f) \right|
    = 
    \left| \text{ev}_{\tilde x} \left( h\circ q \cdot \mu(f) \right) \right|
    =
    \left| \text{ev}_{\tilde x} \left( \theta(h) \cdot \mu(f) \right) \right|
    = 
    \left| \text{ev}_{\tilde x} \left( \mu(f \cdot \theta(h)) \right) \right|
    \leq 
    \left\| f \cdot \theta(h) \right\|
    \leq \eps,
  \end{equation*}
  as $\mu(\theta(h)) = \theta(h)$ is contained in the multiplicative domain
  of $\mu$.
  Now denote by $\mu_{\tilde x}$ the measure on $p^{-1}(x)$
  associated to $\text{ev}_{\tilde x} \circ \mu$.
  As the map is unital, this is a probability measure.

  For every $\gamma \in \G_x^x \setminus \left\{ x \right\}$ pick 
  an open bisection $B_\gamma$ that does not intersect the unit space
  and
  $f_\gamma \in C_c\left( \G \right)$ supported on $B_\gamma$
  such that $f_\gamma(\gamma) = 1$.
  Naturally, $f_\gamma(\gamma') = 0$
  for all $\gamma \neq \gamma' \in \G_x^x$
  while $\mu\circ \theta(f_\gamma) = 0$,
  as this is the canonical expectation.
  Furthermore,  $f_\gamma$ is supported away from the unit space
  and $\theta(f_\gamma)$ restricted to $p^{-1}(x)$
  is the characteristic function of the set
  $\left\{ \Lambda_x \in \Lambda \bigm| \gamma \in \Lambda_x \right\}$.

  Thus we may calculate 
  \begin{align*}
    \mu_{\tilde x}\left( p^{-1}(x) \setminus \left\{ x \right\} \right)
    &\leq
    \sum\limits_{\gamma \in \G_x^x \setminus\left\{ x \right\}}
    \mu_{\tilde x}
    \left(  
      \left\{ \Lambda_x \in \Lambda \bigm| \gamma \in \Lambda_x\right\}
    \right)
    \\
    &= 
    \sum\limits_{\gamma \in \G_x^x \setminus\left\{ x \right\}}
    \mu_{\tilde x}\left( \theta(f_\gamma) \right)
    = 
    \sum\limits_{\gamma \in \G_x^x \setminus\left\{ x \right\}}
    \text{ev}_{\tilde x}\left( \mu\circ\theta(f_\gamma) \right)
    = 
    0.
  \end{align*}
  Hence $\left\{ x \right\} \in p^{-1}(x) \subseteq \Lambda$,
  which is exactly the condition of Proposition \ref{thm:main}.
\end{proof}


